AMREx: AMR for Explainable Fact Verification

With the advent of social media networks and the vast amount of information circulating through them, automatic fact verification is an essential component to prevent the spread of misinformation. It is even more useful to have fact verification systems that provide explanations along with their classifications to ensure accurate predictions. To address both of these requirements, we implement AMREx, an Abstract Meaning Representation (AMR)-based veracity prediction and explanation system for fact verification using a combination of Smatch, an AMR evaluation metric to measure meaning containment and textual similarity, and demonstrate its effectiveness in producing partially explainable justifications using two community standard fact verification datasets, FEVER and AVeriTeC. AMREx surpasses the AVeriTec baseline accuracy showing the effectiveness of our approach for real-world claim verification. It follows an interpretable pipeline and returns an explainable AMR node mapping to clarify the system's veracity predictions when applicable. We further demonstrate that AMREx output can be used to prompt LLMs to generate natural-language explanations using the AMR mappings as a guide to lessen the probability of hallucinations.

==> images/fever_example.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,581); %set diagram left start at 0, and has height of 581

%Shape: Rectangle [id:dp08708278645101009] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (11.98,296.5) -- (59.4,296.5) -- (59.4,326) -- (11.98,326) -- cycle ;

%Shape: Rectangle [id:dp11737779691911288] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (91.45,252.5) -- (113,252.5) -- (113,282) -- (91.45,282) -- cycle ;

%Straight Lines [id:da4900385207658885] 
\draw    (62.92,298.19) -- (88.95,266.81) ;
\draw [shift={(90.86,264.5)}, rotate = 129.68] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
\draw [shift={(61,300.5)}, rotate = 309.68] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Straight Lines [id:da5349686913314947] 
\draw    (63,311.5) -- (86,311.5) ;
\draw [shift={(89,311.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
\draw [shift={(60,311.5)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Straight Lines [id:da4623129531829612] 
\draw    (63.81,324.89) -- (88.19,357.11) ;
\draw [shift={(90,359.5)}, rotate = 232.88] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
\draw [shift={(62,322.5)}, rotate = 52.88] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Shape: Rectangle [id:dp24669933986402748] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (148.65,252.5) -- (168.47,252.5) -- (168.47,282) -- (148.65,282) -- cycle ;

%Shape: Rectangle [id:dp8864681787257874] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (148.7,296.25) -- (169.5,296.25) -- (169.5,325.75) -- (148.7,325.75) -- cycle ;

%Shape: Rectangle [id:dp7272260266067082] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (149.04,340.25) -- (170.49,340.25) -- (170.49,369.75) -- (149.04,369.75) -- cycle ;

%Straight Lines [id:da16607452239947884] 
\draw    (115.1,267.54) -- (145.5,267.96) ;
\draw [shift={(148.5,268)}, rotate = 180.79] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
\draw [shift={(112.1,267.5)}, rotate = 0.79] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Straight Lines [id:da4223831227313489] 
\draw    (117.5,312) -- (143.5,312) ;
\draw [shift={(146.5,312)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
\draw [shift={(114.5,312)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Straight Lines [id:da9718959971214775] 
\draw    (116.5,354) -- (145.5,354) ;
\draw [shift={(148.5,354)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
\draw [shift={(113.5,354)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Rounded Rect [id:dp36530946279971477] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (3.5,269.47) .. controls (3.5,253.19) and (16.7,240) .. (32.97,240) -- (155.41,240) .. controls (171.69,240) and (184.88,253.19) .. (184.88,269.47) -- (184.88,357.87) .. controls (184.88,374.14) and (171.69,387.33) .. (155.41,387.33) -- (32.97,387.33) .. controls (16.7,387.33) and (3.5,374.14) .. (3.5,357.87) -- cycle ;
%Straight Lines [id:da21204352826283812] 
\draw    (253,407.33) -- (253,390.2) ;
\draw [shift={(253,387.2)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp9000697424351067] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (221.96,336.86) -- (283.49,336.86) -- (283.49,388) -- (221.96,388) -- cycle ;

%Straight Lines [id:da8710000736492601] 
\draw    (252.5,337) -- (252.5,307) ;
\draw [shift={(252.5,304)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp0654595191830466] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (220.65,274.86) -- (284.5,274.86) -- (284.5,305) -- (220.65,305) -- cycle ;

%Shape: Rectangle [id:dp7149398606916143] 
\draw   (1.98,0.5) -- (289.64,0.5) -- (289.64,225.78) -- (1.98,225.78) -- cycle ;

%Shape: Rectangle [id:dp037496064612650315] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (91.87,297.25) -- (113.5,297.25) -- (113.5,327) -- (91.87,327) -- cycle ;

%Shape: Rectangle [id:dp8580550214727524] 
\draw  [fill={rgb, 255:red, 169; green, 150; blue, 198 }  ,fill opacity=0.57 ] (91.76,338.25) -- (114.41,338.25) -- (114.41,367.75) -- (91.76,367.75) -- cycle ;

%Straight Lines [id:da6346443921541389] 
\draw    (95.17,387.2) -- (95.59,403.67) ;
\draw [shift={(95.67,406.67)}, rotate = 268.53] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Shape: Rectangle [id:dp702268434061912] 
\draw   (3.5,406.67) -- (283.49,406.67) -- (283.49,446.67) -- (3.5,446.67) -- cycle ;

% Text Node
\draw (35.69,311.25) node   [align=left] {\begin{minipage}[lt]{32.24pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont claim}
\end{center}

\end{minipage}};
% Text Node
\draw (102.22,267.25) node   [align=left] {\begin{minipage}[lt]{14.66pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Q1}
\end{center}

\end{minipage}};
% Text Node
\draw (67.56,264.95) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-358.78] [align=left] {{\fontfamily{ptm}\selectfont E}};
% Text Node
\draw (69.25,295.74) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.75] [align=left] {{\fontfamily{ptm}\selectfont  E}};
% Text Node
\draw (66.97,339.62) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.36] [align=left] {{\fontfamily{ptm}\selectfont E}};
% Text Node
\draw (158.56,267.25) node   [align=left] {\begin{minipage}[lt]{13.48pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont A1}
\end{center}

\end{minipage}};
% Text Node
\draw (159.1,311) node   [align=left] {\begin{minipage}[lt]{14.14pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont A2}
\end{center}

\end{minipage}};
% Text Node
\draw (159.77,355) node   [align=left] {\begin{minipage}[lt]{14.59pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont A3}
\end{center}

\end{minipage}};
% Text Node
\draw (118.83,249.28) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.01] [align=left] {\begin{minipage}[lt]{16.32pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont NE}
\end{center}

\end{minipage}};
% Text Node
\draw (119.71,296) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.01] [align=left] {\begin{minipage}[lt]{16.32pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont NE}
\end{center}

\end{minipage}};
% Text Node
\draw (121,338) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.01] [align=left] {\begin{minipage}[lt]{16.32pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont NE}
\end{center}

\end{minipage}};
% Text Node
\draw (252.73,362.43) node   [align=left] {\begin{minipage}[lt]{41.84pt}\setlength\topsep{0pt}
{\fontfamily{ptm}\selectfont Threshold function}
\end{minipage}};
% Text Node
\draw (252.58,289.93) node   [align=left] {\begin{minipage}[lt]{43.42pt}\setlength\topsep{0pt}
{\fontfamily{ptm}\selectfont Refuting}
\end{minipage}};
% Text Node
\draw (145.82,113.14) node   [align=left] {\begin{minipage}[lt]{196.38pt}\setlength\topsep{0pt}
{\fontfamily{ptm}\selectfont \textbf{Claim:} "45\% of Nigeria's revenue goes to the federal government."}\\\\{\fontfamily{ptm}\selectfont \textbf{Q1:} "How much of Nigeria's revenue goes to the federal government?"}\\{\fontfamily{ptm}\selectfont \textbf{A1: }"52.68 \% goes to the federal government."}\\\\{\fontfamily{ptm}\selectfont \textbf{Q2:} "How much of Nigeria's revenue went to the federal government in 2019?"}\\{\fontfamily{ptm}\selectfont \textbf{A2:} "2,661.13 trillion went to \ federal government from the 5,051.50 trillion available for sharing."}\\\\{\fontfamily{ptm}\selectfont \textbf{Q3:} "What percentage of the revenue in Nigeria goes to the Federal government?"}\\{\fontfamily{ptm}\selectfont \textbf{A3:} "52.68 \% goes to the federal government."}
\end{minipage}};
% Text Node
\draw (102.68,312.13) node   [align=left] {\begin{minipage}[lt]{14.71pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Q2}
\end{center}

\end{minipage}};
% Text Node
\draw (103.08,353) node   [align=left] {\begin{minipage}[lt]{15.4pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Q3}
\end{center}

\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (1.5,399.33) -- (285.5,399.33) -- (285.5,443.33) -- (1.5,443.33) -- cycle  ;
\draw (143.5,421.33) node  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{190.39pt}\setlength\topsep{0pt}

{\footnotesize \begin{equation*}
\frac{(( 1*( -1)) +( 1*( -1)) +( 1*( -1))}{3} =-1
\end{equation*}}
\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (207.89,225.62) -- (299.89,225.62) -- (299.89,256.62) -- (207.89,256.62) -- cycle  ;
\draw (253.89,241.12) node  [font=\small] [align=left] {\begin{minipage}[lt]{59.51pt}\setlength\topsep{0pt}
{\fontfamily{ptm}\selectfont \textcolor[rgb]{0.29,0.56,0.89}{{\scriptsize \textbf{E: Entail (+1)}}}}\\{\fontfamily{ptm}\selectfont \textcolor[rgb]{0.29,0.56,0.89}{{\scriptsize \textbf{NE: Non-Entail (-1)}}}}
\end{minipage}};


\end{tikzpicture}

